Entangling lattice-trapped bosons with a free impurity: impact on stationary and dynamical properties

We address the interplay of few lattice trapped bosons interacting with an impurity atom in a box potential. For the ground state, a classification is performed based on the fidelity allowing to quantify the susceptibility of the composite system to structural changes due to the intercomponent coupling. We analyze the overall response at the many-body level and contrast it to the single-particle level. By inspecting different entropy measures we capture the degree of entanglement and intraspecies correlations for a wide range of intra- and intercomponent interactions and lattice depths. We also spatially resolve the imprint of the entanglement on the one- and two-body density distributions showcasing that it accelerates the phase separation process or acts against spatial localization for repulsive and attractive intercomponent interactions respectively. The many-body effects on the tunneling dynamics of the individual components, resulting from their counterflow, are also discussed. The tunneling period of the impurity is very sensitive to the value of the impurity-medium coupling due to its effective dressing by the few-body medium. Our work provides implications for engineering localized structures in correlated impurity settings using species selective optical potentials.

==> dynamics.tex <==
\section{Quench induced tunneling dynamics}
\label{sec:dyn}

\begin{figure*}[t]
	\includegraphics[width=\textwidth]{densities3.png}
	\caption{(a) One-body density $\rho^{\sigma}_1(x)$ of the initial state configuration for $V=500$, $g_{AA}=0.5$ and $g_{AB}=6.0$ at $t=0$. Temporal evolution of (b) the averaged position of the impurity $\langle\hat{X}_B\rangle$ (see eq. \ref{eq:com}), (c) the one-body density of the majority species and (d) the one-body density of the impurity upon quenching the interspecies interaction strength to $g_{AB}=4.5$. \label{fig:densities}}
\end{figure*}
Having analyzed in detail the ground state properties of our system, we subsequently study the dynamical response of a single impurity coupled to a lattice trapped species upon quenching the interspecies interaction strength $g_{AB}$. To this end we prepare the system in its ground state for $V=500$, $g_{AB}=6.0$ and $g_{AA}=0.5$, leading to the formation of a two-fold degeneracy in the ground state and the two species phase separate. In this sense, the ground state one-body density is given by a superposition state of two parity-symmetry broken configurations, where the density of the first one is depicted in Fig. \ref{fig:densities} (a) and the second one corresponds to its parity-symmetric (with respect to $x = 0$) counterpart.
It is possible to remove this degeneracy in order to select any of the states in the respective degenerate manifold. Technically, this is done by applying a small asymmetry, e.g. a tilt, to the lattice potential, thereby breaking the parity symmetry and energetically favoring one of the above-mentioned states.

To trigger the dynamics starting from the initial state configuration illustrated in Fig. \ref{fig:densities} (a) we quench the interspecies interaction strength to a smaller value. 
As a representative example of the emergent tunneling dynamics of each species we present the temporal evolution of the corresponding one-body densities in Fig. \ref{fig:densities} (c), (d) following a quench to $g_{AB}=4.5$, while keeping fixed $V=500$ and $g_{AA}=0.5$. In this case the impurity performs an oscillatory motion which is reminiscent of the tunneling of a particle in a double-well. This can be attributed to the lifting of the degeneracy for smaller interspecies interaction strengths. For a post-quench strength of $g_{AB}=4.5$ the initially prepared state has a substantial overlap with the post-quench ground state and the first excited state such that in the course of the dynamics the system will oscillate between those two. This is similar to a single particle in a double-well which is prepared as a superposition of the first doublet and undergoes a tunneling between the sites.
Correspondingly, the majority species will undergoes a collective tunneling in the lattice geometry. Thus, the probability distribution of a single majority species particle will oscillate between the initial distribution [Fig. \ref{fig:densities} (a)] and its parity-symmetric counterpart. Due to the repulsive nature of the interspecies coupling the two species move in opposite directions such that they end up in phase-separated configurations after half a period. 
Note that the oscillation period, being the energy gap between the two energetically lowest eigenstates of the post-quench Hamiltonian (not shown here), depends on the post-quench $g_{AB}$. This can be easily verified by monitoring the temporal evolution of the averaged position of the impurity which is defined as 
\begin{equation}
\langle\hat{X}_B\rangle=\int_{-L/2}^{L/2}dx\rho_{1}^{B}(x) x.
\label{eq:com}
\end{equation}
For various post-quench $g_{AB}$ we find that the impurity will occupy its parity-symmetric counterpart, reflected in the decrease of $\langle\hat{X}_B\rangle$ towards negative values, while the oscillation decreases with smaller $g_{AB}$ [Fig. \ref{fig:densities} (b)].  
\begin{figure*}[t]
	\includegraphics[width=0.8\textwidth]{natorb2.png}
	\caption{Temporal evolution of the density of (a) the first and (b) the second natural orbital $\Phi^{B}_j(x,t)$ (see eq. \ref{eq:particle_entropy}) of the impurity and (c), (d) the natural populations $n^{\sigma}_j$ of both subsystems upon quenching the interspecies interaction strength $g_{AB}$ of the ground state in Fig. \ref{fig:densities} (a) to $g_{AB}=4.5$. \label{fig:natorb}}
\end{figure*}

In order to get insight into beyond mean-field effects we investigate the natural populations $n^{\sigma}_j$ (see eq. \ref{eq:particle_entropy}) which indicate the degree of fragmentation of the subsystem.
For simplicity here we present the populations of the first two dominantly populated natural orbitals while using six orbitals in the actual calculations. 
The initial depletion of both subsystems is rather small, i.e. $n^{A}_1\approx0.996$ and $n^{B}_1\approx0.99$, such that any decrease of these populations upon quenching $g_{AB}$ is due to dynamical many-body effects.
We find that for both subsystems dominantly two natural orbitals contribute during the dynamics [Fig. \ref{fig:natorb} (c), (d)], while the ones of the medium are less impacted by the quench. For the natural populations of the impurity signatures of an oscillation can be observed, where $n^B_1$ initially decreases and revives back towards $n^{B}_1\approx0.99$, while $n^B_2$ initially increases and afterwards drops back to nearly zero. In order to attribute the occupation of the additional natural orbital to physical processes, we analyze the spatial distribution of the natural orbitals $\Phi^{B}_j(x,t)$ (see eq. \ref{eq:particle_entropy}) themselves focusing on the impurity [Fig. \ref{fig:natorb} (a), (b)].
In Fig. \ref{fig:natorb} (a) we observe that the first natural orbital corresponds to the oscillatory behavior of the one-body density  of the impurity, but lacking the smooth transition between the phase-separated configurations [see Fig. \ref{fig:densities} (d)]. The first natural orbital dominates during the dynamics and we can interpret its behavior as corresponding to the presence of the phase-separated density configurations. Consequently, the second natural orbital [Fig. \ref{fig:natorb} (b)], resembling the mirror image of the first one, contributes to deviations from this solution. Due to its structure we can deduce that it is responsible for initiating the transport of the impurity, thereby allowing for the counterflow of the two species.
Note that the presence of more than one natural orbital during the dynamcis is a clear signature that mean-field theory would not provide an accurate description of the system dynamics. Hence, the fact that $\ket{\Phi^B_2}$ is occupied is a manifestation of many-body effects, influencing the motion of both species.


%Quenching the interspecies interaction strength we are able to induce a dynamical process which for the impurity is reminiscent of the tunneling of a single particle in a double well potential.
%This can be attributed to the lifting of the quasi-degeneracy for the corresponding post-quench Hamiltonian. Due to the repulsive interspecies interaction also the majority species will undergo a tunneling in the lattice geometry such that the two species move in opposite directions, ending up in phase-separated configurations after half a period.
%We identify the presence of two dominant natural orbitals for the impurity species during the dynamics, where the first one corresponds to the dynamical behavior of the respective one-body density while the second one resembles the mirror image of the first one. The presence of an additional natural orbital emphasizes the many-body character of the dynamics, thereby influencing the motion of the impurity.

==> intro.tex <==
\begin{abstract} 

We address the interplay of few lattice trapped bosons interacting with an impurity atom in a box potential. 
For the ground state, a classification is performed based on the fidelity allowing to quantify the overall disturbance of the composite system due to the introduction of the intercomponent coupling and also to explicate the competition between many-body and single-particle effects. 
Inspecting different entropy measures we capture the degree of entanglement and intraspecies correlations for a wide range of intra- and intercomponent interactions and lattice depths. 
We also spatially resolve the imprint of the entanglement on the one- and two-body density distributions showcasing, in particular, that it accelerates the phase separation process or acts against spatial localization at repulsive and attractive couplings respectively. 
The many-body effects on the tunneling dynamics of the components, resulting from their counterflow, are also discussed with the tunneling period of the impurity being affected by the value of the impurity-medium coupling due to its effective dressing by the few-body medium. 
Our work provides implications for engineering localized structures in correlated impurity settings using species selective optical potentials.

\end{abstract}

\maketitle

\section{Introduction}\label{Intro} 

Multicomponent quantum gases can be experimentally studied with a high degree of controllability in the ultracold regime~\cite{bloch2008many,bloch2017probing}. 
Specifically, both Bose and Fermi mixtures can be trapped in various species selective external geometries~\cite{fukuhara2009all,henderson2009experimental}, few-body ensembles are possible to realize in particular in one-dimension (1D)~\cite{serwane2011deterministic,schmied2016bell} while the scattering lengths are tunable through Feshbach and confinement induced resonances~\cite{chin2010feshbach,kohler2006production}. 
In 1D bosonic mixtures the adjustability of the intercomponent interactions gives rise to intriguing phenomena such as phase-separation processes~\cite{mistakidis2018correlation,pyzh2020phase} in the repulsive regime, formation of bound states, e.g., droplet configurations~\cite{petrov2016ultradilute,parisi2020quantum} for attractive interactions as well as quasiparticle-like states in highly particle imbalanced systems~\cite{catani2012quantum,meinert2017bloch}. 

In this latter context, an impurity species is embedded in a majority environment called the medium. 
The presence of finite impurity-medium coupling leads to an effective picture where the impurity properties deviate from the bare particle case exhibiting, for instance, an effective mass~\cite{mistakidis2019effective,ardila2015impurity,grusdt2017bose} and induced interactions~\cite{dehkharghani2018coalescence,mistakidis2020induced} mediated by the medium. 
The resultant states are often called polarons~\cite{massignan2014polarons,schmidt2018universal} and have been experimentally realized mainly in higher-dimensions~\cite{fukuhara2013u,yan2020bose,scazza2017repulsive,jorgensen2016observation,cetina2016ultrafast} and to a lesser extent in 1D~\cite{catani2012quantum,wenz2013few} using spectroscopic schemes. 
Since these settings consist of a few-body subsystem they naturally show enhanced correlation properties, especially in 1D, rendering their many-body treatment inevitable. 
In particular, the emergent impurity-medium entanglement can lead to spatial undulations of the medium. 
This mechanism is manifested, for instance, as sound-wave emission~\cite{mistakidis2020radiofrequency,grusdt2017bose} and collective excitations~\cite{mistakidis2020many,boudjemaa2020breathing} of the host or the formation of a bound state~\cite{ardila2020strong,camacho2018bipolarons,mukherjee2020induced} between the impurity and atoms of the medium for attractive interspecies interactions. 

Another relevant ingredient here is the type of the external trapping geometry that the two components experience. 
Indeed, for harmonically trapped and homogeneous systems remarkable dynamical features of impurity physics include the spontaneous generation of localized patterns~\cite{bougas2020pattern,grusdt2017bose}, inelastic collisional aspects of driven impurities~\cite{mistakidis2019dissipative,mukherjee2020pulse,theel2020many} with the surrounding and their relaxation at long timescales~\cite{mistakidis2020pump,lausch2018prethermalization,palzer2009quantum}. 
On the other hand, when a lattice potential is introduced the situation becomes more complicated giving rise, among others, to doped insulator physics~\cite{keiler2020doping,bohrdt2020dynamical} and impurity transport~\cite{cai2010interaction,johnson2011impurity,theel2020entanglement}. 
Apparently, configuring one component by manipulating its external trap while leaving the other intact, e.g. by using a species selective external potential, it is possible to control the response of the unperturbed component via the impurity-medium interaction~\cite{keiler2018state,keiler2018correlation}. 
For instance, operating in the lowest-band approximation it has been demonstrated that a lattice trapped impurity interacting with a homogeneous host exhibits besides tunneling dynamics~\cite{keiler2019interaction} also self-trapping events~\cite{bruderer2008self,yin2015polaronic} and can even undergo Bloch-oscillations~\cite{grusdt2014bloch}. 
The opposite case, where the medium resides in the lattice, provides an experimental probe of the impurity-medium collision parameters~\cite{weber2010single} and interaction strength~\cite{will2011coherent}.  

In this work by considering an impurity in a box potential and a lattice trapped few-body medium we examine how the latter affects the impurity's spatial distribution by means of (de-)localization for different lattice depths and intercomponent interactions. 
Indeed, a lattice trapped medium can reside either in a superfluid or an insulating-like phase~\cite{keiler2020doping}, a fact that is expected to crucially impact the impurity's configuration and vice versa. 
To address the ground state properties and quantum quench dynamics of the above-discussed impurity setting we utilize the multi-layer multi-configuration time-dependent Hartree method for atomic mixtures (ML-MCTDHX)~\cite{cao2017unified,cao2013multi,kronke2013non}. 
This variational method enables us to account for the relevant correlations of the mixture and operate beyond the lowest-band approximation for the medium. 

Focusing on the ground state of the system and in order to testify its overall response for varying intercomponent interactions we calculate the fidelity between the coupled and decoupled composite system both at the many-body and the single-particle level. 
Note that in impurity settings this observable is commonly termed residue~\cite{massignan2014polarons,schmidt2018universal} enabling us to identify e.g. the polaron formation, while the influence of the impurity-medium entanglement in this observable is still an open issue. 
It is demonstrated that despite the fact that the total entangled state may strongly deviate from its decoupled configuration, this effect is arguably less pronounced or even diminished at the single-particle level. 
Furthermore, we showcase that the build-up of impurity-medium entanglement is sensitive to the interplay between the intercomponent interactions and the lattice depth~\cite{keiler2020doping}. 
Interestingly, stronger interactions do not necessarily lead to a larger amount of entanglement, whereas the state of the majority species may undergo substantial structural changes, which remain invisible at the single-particle level. 
Moreover, we identify the imprint of the background on the impurities and vice versa by relying on one- and two-body density distributions evincing a rich spatial structure of the components with respect to the lattice depth as well as the inter- and intra-component interactions. 
In particular, it is argued that for repulsive (attractive) interactions the impurity delocalizes (localizes) around the central lattice site. 
The delocalization of the impurity is accompanied by its phase-separation with the majority component~\cite{mistakidis2019quench}, where the impurity tends to the edges of the box for a superfluid background or exhibits a multi-hump structure for an insulating medium. 
Deviations of the previous configurations when considering a state ignoring entanglement effects are spatially resolved in terms of the one- and two-body densities demonstrating that entanglement favors phase-separation and generally inhibits spatial localization at positive and attractive couplings respectively. 

Furthermore, we monitor the non-equilibrium dynamics of the mixture. 
In particular, we prepare the system in a phase-separated, i.e. disentangled configuration, and quench the intercomponent interactions to smaller values resulting in the counterflow of the components and thus triggering their tunneling dynamics and the consequent build-up of entanglement. 
The majority component plays the role of a material barrier for the impurity~\cite{theel2020entanglement,pflanzer2009material} which performs tunneling oscillations  
whose period depends strongly on the impurity-medium interaction. 
The many-body nature of the tunelling process of the components is testified by invoking the individual natural orbitals constituting the time-evolved many-body state. 

Our presentation is structured as follows. 
In \cref{sec:setup} we introduce the considered impurity setting 
and in \cref{sec:methodology} we discuss our 
many-body treatment to tackle its ground state and dynamics. 
The ground state properties of the delocalized impurity 
and the lattice trapped medium are addressed in \cref{sec:ground_state}. 
In particular, we analyze the fidelity between perturbed and unperturbed (reduced) density operators, quantify the degree of entanglement and visualize its impact on single- and two-body density distributions of each species for different intra- and intercomponent interactions and lattice depths. 
The non-equilibrium dynamics of the mixture after a quench of the impurity-medium coupling to smaller values is discussed in \cref{sec:dyn}. 
We provide a summary of our results and elaborate on future perspectives in \cref{sec:summary}. 

